A note on joint calibration estimators for totals and quantiles

In this paper, we combine calibration for population totals proposed by Deville and S\"arndal (1992) with calibration for population quantiles introduced by Harms and Duchesne (2006). We also extend the pseudo-empirical likelihood method proposed by Chen, Sitter, and Wu (2002). This approach extends the calibration equations for totals by adding relevant constraints on quantiles of continuous variables observed in the data. The proposed approach can be easily applied to handle non-response and data integration problems, and results in a single vector of weights. Furthermore, it is a multipurpose solution, i.e. it makes it possible to improve estimates of means, totals and quantiles for a variable of interest in one step. In a limited simulation study, we compare the proposed joint approach with standard calibration, calibration using empirical likelihood and the correctly specified inverse probability weighting estimator. Open source software implementing the proposed method is available.

==> Starocie.tex <==
\subsection{Notation}

In the notation, we follow \citet{yang2021integration}. Let $\mathcal{F}_{N}=\left\{\left(\bX_{i}, Y_{i}\right): i \in \Omega \right\}$ with $\Omega=\{1, \ldots, N\}$ denote a finite population, where $\bX_{i}=\left(X_{i}^{1}, \ldots, X_{i}^{p}\right)$ is a $p$-dimensional vector of covariates, and $Y_{i}$ is the study (target) variable. We assume that $\mathcal{F}_{N}$ is a random
sample from a superpopulation model $\zeta$, and $N$ is known. Our objective is to estimate the general finite
population parameter $\mu_{g}=N^{-1} \sum_{i \in \Omega} g\left(Y_{i}\right)$ for some known $g(\cdot)$. For example, if $g(Y)=Y$, $\mu_g=N^{-1}\sum_{i \in \Omega}Y_i$ is the population mean of Y or if $g(Y)$ is given by


\begin{equation}
    g(Y) = \text{inf}(t|F_Y(t) \geq \alpha),
\end{equation}

\noindent where $\alpha \in (0,1), t \in \mathbb{R}$ and $F_y$ can be distribution function (if known)

$$
F_{Y}(t)=\frac{\sum_{i \in \Omega} H\left(t-Y_{i}\right)}{N}, \quad \text{where } H\left(t-Y_{i}\right)=\left\{\begin{array}{ll}1, & t \geqslant Y_{i} \\ 0, & t<Y_{i}\end{array}\right.,
$$

\noindent for $i=1,\ldots, N$, $t \in \mathbb{R}$.

If probability sample $s$ of size $n$ is available, \citet{harms2006calibration} proposed a~lineary interpolated $H_{Y, s}$ which leads to interpolated distribution function given by

$$
\hat{F}_{Y,d}(t)=\frac{\sum_{i \in s} d_{i} H_{Y, s}\left(t, Y_{i}\right)}{\sum_{i \in s} d_{i}}, 
$$

\noindent where function $H_{Y, s}\left(t, Y_{i}\right)$ is given by

$$
H_{Y, s}\left(t, Y_{i}\right)=\left\{
\begin{array}{ll}
1, & Y_{i} \leqslant L_{Y, s}(t) \\ 
\beta_{Y, s}(t), & Y_{i}=U_{Y, s}(t) \\ 
0, & Y_{i}>U_{Y, s}(t)
\end{array}\right.,
$$

\noindent where 

$$
\begin{array}{c}
L_{Y, s}(t)=\max \left\{\left\{Y_{i}, i \in s \mid Y_{i} \leqslant t\right\} \cup\{-\infty\}\right\}, \\ 
U_{Y, s}(t)=\min \left\{\left\{Y_{i}, i \in s \mid Y_{i}>t\right\} \cup\{\infty\}\right\}, \\ 
\beta_{Y, s}(t)=\frac{t-L_{Y, s}(t)}{U_{Y, s}(t)-L_{Y, s}(t)},
\end{array}
$$

\noindent for $i =1,...,n$, $t \in \mathbb{R}$.

In this setting, we can define interpolated distribution function for the auxiliary variable $X_p$ given by

$$
\hat{F}_{X_p, d}(t)=\frac{\sum_{i \in s} d_{i} H_{X_p, s}\left(t, X_{pi}\right)}{\sum_{i \in s} d_{i}}, 
$$

\noindent where $H_{X_p, s}\left(t, X_{ip}\right)$ is defined as

$$
H_{X_p, s}\left(t, X_{pi}\right)=\left\{
\begin{array}{ll}
1, & X_{ip} \leqslant L_{X_p, s}(t) \\ \beta_{X_p, s}(t), & X_{ip}=U_{X_p, s}(t) \\ 0, & X_{ip}>U_{X_p, s}(t)
\end{array}\right.,
$$

\noindent where 

$$
\begin{array}{c}
L_{X_p, s}(t)=\max \left\{\left\{X_{pi}, i \in s \mid X_{pi} \leqslant t\right\} \cup\{-\infty\}\right\} \\ 
U_{X_p, s}(t)=\min \left\{\left\{X_{pi}, i \in s \mid X_{pi}>t\right\} \cup\{\infty\}\right\} \\ 
\beta_{X_p, s}(t)=\frac{t-L_{X_p, s}(t)}{U_{X_p, s}(t)-L_{X_p, s}(t)}
\end{array},
$$

\noindent for $i =1,...,n$, $t \in \mathbb{R}$. If calibration weights $w_i$ then they can replace design-based weights $d_i$ in the 
 
Under such setting $\mu_{g, \alpha} = F_Y^{-1}(\alpha)$ is $\alpha$ quantile of $Y$ variable in the population.

%% notation for non-probability samples

\subsection{Calibration for totals}

%% Marcin, tu o kalibracji ogolnie, krótko i zwięzle

$$
\mu_gN=\sum_{i \in s} w_{i} y_{i},
$$

$$
D(\bd, \bw)=\sum_{i \in s} \frac{d_{i}}{q_{i}} G\left(\frac{w_{i}}{d_{i}}\right) \rightarrow \min
$$

$$
\sum_{i \in s} w_{i} \bx_{i}=\sum_{i \in \Omega} \bx_{i} = \btau
$$

\noindent or if totals are estimated

$$
\sum_{i \in s} w_{i} \bx_{k}=\hat{\btau},
$$

\noindent with possible restrictions on weights dispersion

\begin{equation}
L \leq \frac{w_{i}}{d_{i}} \leq U, \text { where: } \quad 0 \leq L \leq 1 \leq U, i=1, \ldots, n
\label{eq-restrictions}
\end{equation}



\subsection{Calibration for quantiles}

%% Marcin, tu o kalibracji ogolnie, krótko i zwięzle

$$
\mu_{g, \alpha}=\hat{F}_{y, c a l}^{-1}(\alpha)
$$

$$
\bw=\argmin_{\bv} D(\bv, \bd)
$$

\begin{equation}
  \begin{array}{c}
\sum_{i \in s} w_{i}=N \\ 
\hat{F}_{x_{i}, \text{CAL}}\left(\mu_{g, \alpha}\right)=\alpha.
\end{array}  
\label{eq-calconst-quantile}
\end{equation}


Alternatively, calibration constraints \eqref{eq-calconst-quantile} can be written as 

\begin{equation}
  \begin{array}{c}
\sum_{i \in s} w_{i}=N \\ 
\sum_{i \in s} w_i a_{i} =\alpha,
\end{array}  
\label{eq-calconst-quantile-alt}
\end{equation}

\noindent where

$$
a_{i j}=
\begin{cases}N^{-1}, &  x_{i j} \leqslant L_{x_{j}, r}\left(\mu_{g, \alpha}\right) \\ 
N^{-1} \beta_{x_{j}, r}\left(\mu_{g, \alpha}\right), & x_{i j}=U_{x_{j}, r}\left(\mu_{g, \alpha}\right) \\ 0, & x_{i j}>U_{x_{j}, r}\left(\mu_{g, \alpha}\right)
\end{cases}
$$

In the next section, we combine calibration estimators for totals and quantiles via calibration constraints. 



\textbf{Remark 1}: As the proposed method is based on calibration it can be easily extended for the generalized calibration, in particular for not missing at random non-response. In generalized calibration we have two set of variables: instrumental ($\bZ$) connected with the response mechanism and auxiliary variables ($\bX$, in our case $\bH$). Using the  

$$
\sum_{i \in r} \bh_kd_i\mathcal{F}(\bgamma^T\bz_i) = \sum_{i \in \Omega} \bh_i,
$$


\noindent where $\bz_i$ is not necessary equal to $\bh_i$, but $\bz_i$ and $\bh_i$ have to be highly correlated and $\bz_i$ should be known for only for respondents denoted as $r$.

\textbf{Remark 2}: The proposed method can be easily applied for household surveys where integrated calibration is applied, i.e. when the weights of household members should be equal. This may be in particular important for EU-SILC where information from admin data may be used to provide population distribution for auxiliary variables.

\textbf{Remark 3}: The proposed method may be unstable for some cases where population totals of $\bX$ are very large (e.g. in millions) in comparison to $\balpha$ that are between $(0,1)$. One may overcome this issue during the numerical procedure by dividing the population size, matrix $\bX$ and $\btau$ by some arbitrary quantity (say 1,000 or 100,000) and multiplying $\bA$ and $\balpha$ by the same quantity. If the method is applied for correcting non-response when the estimated distribution of some variable $\bx$ is available then one may consider using scaled (standardized) variables instead.   

\textbf{Remark 4}: The proposed method can be easily implemented in existing statistical packages such as \texttt{survey} in R, \texttt{samplics} in Python or \texttt{svyset} in Stata. This allows the researcher to specify distance functions (e.g. raking, logit or hyperbolic sinus), to control the spread of weights or to perform trimming of extreme weights. Example codes are presented in the Supplementary Materials.

% \section{Additional simulation studies}

% \subsection{JOS 2016}

% \begin{table}[ht]
% \centering
% \small
% \begin{tabular}{lllrrrrrrrr}
%   \hline
% dist & resp & type & y1\_rb & y1\_rmse & y2\_rb & y2\_rmse & y3\_rb & y3\_rmse & y4\_rb & y4\_rmse \\ 
%   \hline
% linear & p1 & CAL & 0.00 & 10.62 & -0.19 & 20.07 & -0.31 & 0.01 & 0.18 & 21.59 \\ 
%        &  & QCAL1 & -0.08 & 10.85 & -1.42 & 13.35 & -0.72 & 0.01 & 0.09 & 11.42 \\ 
%        &  & QCAL2 & -0.00 & 10.79 & -0.43 & 12.06 & -0.21 & 0.01 & 0.38 & 12.10 \\ 
%        & p2 & w0 & -0.03 & 10.86 & -4.27 & 24.76 & -3.01 & 0.01 & 3.04 & 32.61 \\ 
%        &  & w1 & -0.12 & 11.12 & -2.04 & 15.30 & -0.84 & 0.01 & 0.36 & 11.66 \\ 
%        &  & w2 & -0.03 & 11.01 & -1.05 & 13.51 & -0.29 & 0.01 & 0.72 & 13.05 \\ 
%        & p3 & w0 & 0.00 & 11.90 & -12.75 & 45.16 & -15.27 & 0.04 & 10.95 & 97.77 \\ 
%        &  & w1 & -0.15 & 12.96 & -2.02 & 17.03 & -1.19 & 0.01 & 0.47 & 12.95 \\ 
%        &  & w2 & -0.04 & 12.84 & -1.25 & 15.73 & -0.71 & 0.01 & 1.07 & 15.76 \\ 
%        &  p4 & w0 & 0.12 & 13.96 & 27.61 & 132.32 & 19.64 & 0.08 & -36.76 & 207.10 \\ 
%        &  & w1 & -0.01 & 16.79 & 1.30 & 17.86 & 0.52 & 0.01 & -1.13 & 18.42 \\ 
%        & & w2 & 0.07 & 16.78 & 3.08 & 21.20 & 0.93 & 0.01 & -1.24 & 19.04 \\ 
%   raking & p1 & w0 & -0.03 & 10.75 & 2.93 & 22.55 & 2.00 & 0.01 & -2.28 & 26.60 \\ 
%        &  & w1 & -0.13 & 11.04 & -1.50 & 13.74 & -0.61 & 0.01 & 0.03 & 10.69 \\ 
%        &  & w2 & -0.04 & 10.90 & -0.04 & 12.02 & 0.04 & 0.01 & 0.09 & 10.90 \\ 
%        & p2 & w0 & -0.08 & 11.29 & 0.22 & 20.60 & 0.18 & 0.01 & -0.07 & 21.12 \\ 
%        &  & w1 & -0.19 & 11.62 & -1.89 & 14.86 & -0.68 & 0.01 & 0.28 & 11.91 \\ 
%        &  & w2 & -0.09 & 11.42 & -0.24 & 12.69 & 0.04 & 0.01 & 0.34 & 12.21 \\ 
%        & p3 & w0 & 0.04 & 12.10 & -0.98 & 25.32 & -6.70 & 0.02 & 4.37 & 42.49 \\ 
%        &  & w1 & -0.14 & 12.83 & -2.30 & 17.49 & -1.33 & 0.01 & 0.52 & 13.73 \\ 
%        &  & w2 & -0.02 & 12.75 & -0.39 & 14.84 & -0.48 & 0.01 & 0.60 & 14.22 \\ 
%        & p4 & w0 & 0.14 & 13.99 & 28.27 & 136.45 & 19.88 & 0.08 & -37.63 & 210.73 \\ 
%        &  & w1 & -0.03 & 16.42 & 1.78 & 17.89 & 0.31 & 0.01 & -0.93 & 18.42 \\ 
%        &  & w2 & 0.05 & 16.44 & 2.91 & 19.69 & 0.81 & 0.01 & -0.92 & 18.42 \\ 
%   logit & p1 & w0 & -0.00 & 10.96 & 2.37 & 21.19 & 1.61 & 0.01 & -1.91 & 24.43 \\ 
%    &  & w1 & -0.10 & 11.14 & -1.52 & 13.79 & -0.64 & 0.01 & 0.06 & 10.73 \\ 
%    &  & w2 & -0.02 & 11.06 & -0.14 & 12.03 & -0.02 & 0.01 & 0.14 & 10.96 \\ 
%    & p2 & w0 & 0.02 & 10.46 & -0.74 & 20.87 & -0.53 & 0.01 & 0.45 & 20.93 \\ 
%    &  & w1 & -0.09 & 10.67 & -2.16 & 15.14 & -0.80 & 0.01 & 0.24 & 11.65 \\ 
%    &  & w2 & 0.01 & 10.63 & -0.61 & 12.74 & -0.08 & 0.01 & 0.34 & 12.03 \\ 
%    & p3 & w0 & 0.04 & 11.81 & -2.75 & 26.55 & -7.56 & 0.02 & 5.29 & 48.69 \\ 
%    &  & w1 & -0.12 & 12.51 & -2.27 & 17.59 & -1.20 & 0.01 & 0.51 & 13.49 \\ 
%    &  & w2 & -0.01 & 12.40 & -0.58 & 14.98 & -0.40 & 0.01 & 0.68 & 14.27 \\ 
%    & p4 & w0 & 0.07 & 13.80 & 27.98 & 134.48 & 19.70 & 0.08 & -37.25 & 208.95 \\ 
%    &  & w1 & -0.12 & 16.87 & 1.51 & 17.53 & 0.33 & 0.01 & -1.01 & 18.76 \\ 
%    &  & w2 & -0.03 & 16.63 & 2.69 & 19.26 & 0.80 & 0.01 & -1.01 & 18.76 \\ 
%    \hline
% \end{tabular}
% \end{table}

% \subsection{\citet{kim2019sampling} example}

% We use the simulation example in \cite{kim2019sampling} to compare various estimators similarly as \cite{yang2021integration}. We generate
% $\left\{\mathbf{X}_{i}=\left(X_{1 i}, X_{2 i}\right), \mathbf{Y}_{i}=\left(Y_{1 i}, Y_{2 i}\right): i=1, \ldots, N\right\}$ with size $N=100,000$, where $Y_{1 i}$ is a~continuous
% outcome and $Y_{2 i}$ is a~binary outcome. From the finite population, we select a~big data sample $B$ where the
% inclusion indicator $\delta_{B i} \sim \operatorname{Ber}\left(p_{i}\right)$ with $p_{i}$ the inclusion probability for unit $i$ with the sample size around 70,000. We obtain a~representative sample $A$ of size $n=1,000$ using simple random sampling. The parameters of interest are the population mean of $Y_1$, population proportion of $Y_2=1$ and quartiles of $Y_1$ (25\%, 50\%, and 75\%).

% For generating the finite population, we consider linear models generating $Y_{11}, Y_{21}$

% $$
% \begin{array}{c}
% Y_{11i} =1+X_{1 i}+X_{2 i}+\alpha_{i}+\varepsilon_{i}, \\ 
% P\left(Y_{21i}=1 \mid X_{1 i}, X_{2 i} ; \alpha_{i}\right)=\logit\left(1+X_{1 i}+X_{2 i}+\alpha_{i}\right),
% \end{array}
% $$

% and non-linear models $Y_{12}, Y_{22}$

% $$
% \begin{array}{c}
% Y_{12i}=0.5\left(X_{1 i}-1.5\right)^{2}+X_{2 i}^{2}+\alpha_{i}+\varepsilon_{i} \\
% P\left(Y_{22i}=1 \mid X_{1 i}, X_{2 i} ; \alpha_{i}\right)=\logit\left\{0.5\left(X_{1 i}-1.5\right)^{2}+X_{2 i}^{2}+\alpha_{i}\right\},
% \end{array}
% $$

% \noindent where \(X_{1 i} \sim \mathcal{N}(1,1), X_{2 i} \sim \Exp(1), \alpha_{i} \sim \mathcal{N}(0,1), \varepsilon_{i} \sim \mathcal{N}(0,1)\), and \(X_{1 i}, X_{2 i}, \alpha_{i}\) and \(\varepsilon_{i}\) are
% mutually independent. The variables \(\alpha_{i}\) induce the dependence of \(Y_{1 i}\) and \(Y_{2 i}\) even adjusting for \(X_{1 i}\) and
% \(X_{2 i}\). For the big-data inclusion probability, we also consider a~logistic linear model  $p_{1}, p_{2}$

% $$
% \logit\left(p_{1i}\right)=X_{2 i},
% $$

% \noindent and non-linear logistic regression

% $$
% \operatorname{logit}\left(p_{2i}\right)=-3+\left(X_{1 i}-1.5\right)^{2}+\left(X_{2 i}-2\right)^{2}.
% $$

% We compare the following estimators

% \begin{enumerate}
%     \item $\hat{\mu}_{\text{Naive}}$ -- sample mean or quantile based on sample B (without correction),
%     \item $\hat{\mu}_{IPW}$ -- we use $X_1$ and $X_2$ assuming logistic linear regression with calibration constraints (as in \citet[sec 3.1]{chen2020doubly}),
%     \item $\hat{\mu}_{KNN}$ -- mass imputation based on $X_1$ and $X_2$ with $k=5$ neighbours,
%     \item $\hat{\mu}_{DR}$ -- we use $X_1$ and $X_2$ assuming linear regression and logistic linear regression  (as in \citet[sec 3.3]{chen2020doubly}),
%     \item $\hat{\mu}_{CAL}$ -- calibration using population size $N$, totals of $X_1$ and $X_2$ variables ($\btau = (N, \tau^{X_1}, \tau^{X_2})^T$),
%     \item $\hat{\mu}_{QCAL1}$ -- calibration using quartiles for $\balpha^{X_1}$ and $\balpha^{X_2}$,
%     \item $\hat{\mu}_{QCAL2}$ -- calibration using totals ($\btau$) and quartiles ($\balpha^{X_1}$ and $\balpha^{X_2}$).
% \end{enumerate}

% Note that for quartiles for DR and IPW we use IPW weights to calculate weighted quartiles. For MI we calculate unweighted quartiles based on imputed $Y$ observations.

% Table \ref{tab-sim2-results-means} presents results for means and Table \ref{tab-sim2-results-quartiles} for quartiles under four scenarios. Plots from the simulations are presented in the Supplementary Materials.

% \begin{table}[ht]
% \centering
% \small
% \caption{Simulation results for means: bias, variance and RMSE under four scenarios based on 1,000 Monte Carlo samples. OM: outcome model, PS: propensity score (all numbers multiplied by 100)}
% \label{tab-sim2-results-means}
% \begin{tabular}{lrrrrrrrrrrrr}
%   \hline 
%   OM & \multicolumn{3}{c}{Linear} & \multicolumn{3}{c}{Linear} & \multicolumn{3}{c}{Nonlinear} & \multicolumn{3}{c}{Nonlinear} \\
%   PS & \multicolumn{3}{c}{Linear} & \multicolumn{3}{c}{Nonlinear} & \multicolumn{3}{c}{Linear} & \multicolumn{3}{c}{Nonlinear} \\
%   Est & Bias & SE & RMSE & Bias & SE & RMSE & Bias & SE & RMSE & Bias & SE & RMSE \\
%   \hline 
%   \multicolumn{13}{c}{Mean of $Y1$} \\
%   \hline
% $\hat{\mu}_{\text{Naive}}$ & 18.87 & 0.37 & 0.19 & -41.13 & 0.45 & 0.41 & 60.89 & 0.59 & 0.61 & 31.13 & 0.83 & 0.32 \\ 
% $\hat{\mu}_{IPW}$ & -0.58 & 5.89 & 0.59 & 68.94 & 28.47 & 2.93 & -0.08 & 10.12 & 1.01 & 450.69 & 170.93 & 17.68 \\ 
% $\hat{\mu}_{KNN}$ & -0.12 & 5.03 & 0.50 & -0.19 & 4.98 & 0.50 & -0.22 & 15.10 & 1.51 & -0.23 & 15.09 & 1.51 \\ 
% $\hat{\mu}_{DR}$ & -0.11 & 4.58 & 0.46 & -0.05 & 4.63 & 0.46 & 1.87 & 6.00 & 0.60 & 217.15 & 72.48 & 7.57 \\ 
% $\hat{\mu}_{CAL}$ & 12.68 & 1.53 & 0.20 & -22.08 & 2.00 & 0.30 & 7.24 & 11.06 & 1.11 & 60.82 & 12.09 & 1.35 \\ 
% $\hat{\mu}_{QCAL1}$ & 1.61 & 4.10 & 0.41 & 19.85 & 4.40 & 0.48 & 9.14 & 8.98 & 0.90 & 150.99 & 12.50 & 1.96 \\ 
% $\hat{\mu}_{QCAL2}$ & -0.11 & 4.59 & 0.46 & -0.11 & 4.60 & 0.46 & -2.64 & 14.26 & 1.43 & 25.83 & 14.03 & 1.43 \\ 
%  \hline 
%   \multicolumn{13}{c}{Mean of $Y2$} \\
%   \hline
% $\hat{\mu}_{\text{Naive}}$ & 1.04 & 0.07 & 0.01 & -4.14 & 0.07 & 0.04 & 2.79 & 0.09 & 0.03 & -1.35 & 0.12 & 0.02 \\ 
% $\hat{\mu}_{IPW}$ & -0.07 & 0.49 & 0.05 & 0.34 & 0.72 & 0.07 & -0.06 & 0.82 & 0.08 & 2.38 & 1.33 & 0.13 \\ 
% $\hat{\mu}_{KNN}$ &  0.00 & 0.55 & 0.06 & -0.02 & 0.54 & 0.05 & -0.06 & 0.79 & 0.08 & -0.01 & 0.81 & 0.08 \\ 
% $\hat{\mu}_{DR}$ & -0.01 & 0.34 & 0.03 & 0.07 & 0.35 & 0.03 & 0.09 & 0.43 & 0.04 & 3.31 & 0.46 & 0.06 \\ 
% $\hat{\mu}_{CAL}$ & 0.93 & 0.13 & 0.02 & -2.88 & 0.15 & 0.03 & 1.01 & 0.44 & 0.05 & -1.39 & 0.31 & 0.03 \\ 
% $\hat{\mu}_{QCAL1}$  & 0.05 & 0.29 & 0.03 & 0.09 & 0.27 & 0.03 & 0.14 & 0.51 & 0.05 & 0.47 & 0.48 & 0.05 \\ 
% $\hat{\mu}_{QCAL2}$ & 0.02 & 0.32 & 0.03 & -0.28 & 0.30 & 0.03 & 0.08 & 0.52 & 0.05 & -0.25 & 0.50 & 0.05 \\ 
%    \hline 
% \end{tabular}
% \end{table}


% \begin{table}[ht]
% \centering
% \small
% \caption{Simulation results for quartiles: bias, variance and RMSE under four scenarios based on 1,000 Monte Carlo samples. OM: outcome model, PS: propensity score (all numbers multiplied by 100)}
% \label{tab-sim2-results-quartiles}
% \begin{tabular}{lrrrrrrrrrrrr}
%   \hline 
%   OM & \multicolumn{3}{c}{Linear} & \multicolumn{3}{c}{Linear} & \multicolumn{3}{c}{Nonlinear} & \multicolumn{3}{c}{Nonlinear} \\
%   PS & \multicolumn{3}{c}{Linear} & \multicolumn{3}{c}{Nonlinear} & \multicolumn{3}{c}{Linear} & \multicolumn{3}{c}{Nonlinear} \\
%   Est & Bias & SE & RMSE & Bias & SE & RMSE & Bias & SE & RMSE & Bias & SE & RMSE \\
% \hline
%   \multicolumn{13}{c}{1$^{th}$ Quartile (25\%) of $Y1$} \\
%   \hline
% $\hat{\mu}_{\text{Naive}}$ & 14.96 & 0.57 & 0.16 & -50.75 & 0.52 & 0.51 & 20.52 & 0.66 & 0.22 & -9.45 & 0.64 & 0.11 \\ 
% $\hat{\mu}_{IPW}$ & -0.77 & 6.26 & 0.63 & 6.56 & 11.92 & 1.19 & -0.32 & 5.72 & 0.57 & 13.52 & 10.01 & 1.01 \\ 
% $\hat{\mu}_{KNN}$ & 30.28 & 5.85 & 0.66 & 30.18 & 5.77 & 0.65 & 21.98 & 4.64 & 0.51 & 22.00 & 4.89 & 0.54 \\ 
% $\hat{\mu}_{DR}$ & -0.77 & 6.26 & 0.63 & 6.56 & 11.92 & 1.19 & -0.32 & 5.72 & 0.57 & 13.52 & 10.01 & 1.01 \\ 
% $\hat{\mu}_{CAL}$ & 12.78 & 1.57 & 0.20 & -37.18 & 1.72 & 0.41 & 7.29 & 3.10 & 0.32 & -10.34 & 1.91 & 0.22 \\ 
% $\hat{\mu}_{QCAL1}$ & 0.69 & 3.95 & 0.40 & -0.99 & 3.64 & 0.36 & 0.94 & 3.49 & 0.35 & 0.26 & 3.36 & 0.34 \\ 
% $\hat{\mu}_{QCAL2}$ & 0.23 & 4.15 & 0.42 & -5.81 & 3.79 & 0.38 & 0.66 & 3.52 & 0.35 & -3.74 & 3.34 & 0.34 \\ 
%    \hline 
%   \multicolumn{13}{c}{2$^{th}$ Quartile (50\%) of $Y1$} \\
%   \hline
% $\hat{\mu}_{\text{Naive}}$ & 17.70 & 0.51 & 0.18 & -49.91 & 0.54 & 0.50 & 31.79 & 0.60 & 0.32 & -12.78 & 0.64 & 0.14 \\ 
% $\hat{\mu}_{IPW}$ & -0.54 & 6.08 & 0.61 & 32.32 & 20.69 & 2.09 & -0.18 & 7.99 & 0.80 & 36.97 & 24.11 & 2.44 \\ 
% $\hat{\mu}_{KNN}$ & -3.91 & 5.83 & 0.58 & -4.24 & 5.85 & 0.59 & -23.81 & 6.75 & 0.72 & -23.68 & 6.77 & 0.72 \\ 
% $\hat{\mu}_{DR}$ & -0.54 & 6.08 & 0.61 & 32.32 & 20.69 & 2.09 & -0.18 & 7.99 & 0.80 & 36.97 & 24.11 & 2.44 \\ 
% $\hat{\mu}_{CAL}$ & 13.46 & 1.49 & 0.20 & -33.38 & 1.78 & 0.38 & 10.86 & 4.93 & 0.50 & -12.86 & 2.90 & 0.32 \\ 
% $\hat{\mu}_{QCAL1}$  & 1.20 & 4.11 & 0.41 & 4.24 & 4.16 & 0.42 & 1.72 & 5.42 & 0.54 & 8.66 & 5.41 & 0.55 \\ 
% $\hat{\mu}_{QCAL2}$ & 0.28 & 4.34 & 0.43 & -6.28 & 4.10 & 0.41 & 0.93 & 5.51 & 0.55 & 0.46 & 5.41 & 0.54 \\ 
%  \hline 
%   \multicolumn{13}{c}{3$^{th}$ Quartile (75\%) of $Y1$} \\ 
%   \hline
% $\hat{\mu}_{\text{Naive}}$ & 21.37 & 0.45 & 0.22 & -44.54 & 0.76 & 0.45 & 66.69 & 0.92 & 0.67 & -17.87 & 0.98 & 0.20 \\ 
% $\hat{\mu}_{IPW}$ & -0.59 & 5.86 & 0.59 & 96.77 & 42.45 & 4.35 & -0.12 & 12.96 & 1.30 & 305.46 & 256.36 & 25.82 \\ 
% $\hat{\mu}_{MI}$ & -36.94 & 7.11 & 0.80 & -36.43 & 7.09 & 0.80 & -42.14 & 15.07 & 1.56 & -41.33 & 15.54 & 1.61 \\ 
% $\hat{\mu}_{DR}$ & -0.59 & 5.86 & 0.59 & 96.77 & 42.45 & 4.35 & -0.12 & 12.96 & 1.30 & 305.46 & 256.36 & 25.82 \\ 
% $\hat{\mu}_{CAL}$ & 13.27 & 1.78 & 0.22 & -22.13 & 2.66 & 0.35 & 17.80 & 10.08 & 1.02 & -10.47 & 7.41 & 0.75 \\ 
% $\hat{\mu}_{QCAL1}$ & 1.80 & 4.38 & 0.44 & 25.02 & 5.63 & 0.62 & 5.25 & 10.20 & 1.02 & 68.45 & 15.18 & 1.67 \\ 
% $\hat{\mu}_{QCAL2}$ & -0.09 & 4.89 & 0.49 & -0.73 & 5.56 & 0.56 & 1.31 & 11.01 & 1.10 & 24.17 & 13.38 & 1.36 \\ 
%    \hline
% \end{tabular}
% \end{table}


% \section{Implementation in R, Python and Stata}

% \subsection{R}

% \subsection{Python}

% \subsection

\begin{equation}
    \begin{aligned}
        \text{Bias}  & = \bar{\hat{\mu}} - \mu,\\
        \text{Standard error (SE)}  & = \sqrt{\frac{\sum_{r=1}^R \left(\hat{\mu}^{(r)} - \bar{\hat{\mu}}\right)^2}{R-1}},\\
        \text{RMSE} & = \sqrt{ \text{Bias}^2 + \text{SE}^2},
    \end{aligned}
    \label{eq-metrics}
\end{equation}
